Foundation Models for Spatio-Temporal Data Science: A Tutorial and Survey

Spatio-Temporal (ST) data science, which includes sensing, managing, and mining large-scale data across space and time, is fundamental to understanding complex systems in domains such as urban computing, climate science, and intelligent transportation. Traditional deep learning approaches have significantly advanced this field, particularly in the stage of ST data mining. However, these models remain task-specific and often require extensive labeled data. Inspired by the success of Foundation Models (FM), especially large language models, researchers have begun exploring the concept of Spatio-Temporal Foundation Models (STFMs) to enhance adaptability and generalization across diverse ST tasks. Unlike prior architectures, STFMs empower the entire workflow of ST data science, ranging from data sensing, management, to mining, thereby offering a more holistic and scalable approach. Despite rapid progress, a systematic study of STFMs for ST data science remains lacking. This survey aims to provide a comprehensive review of STFMs, categorizing existing methodologies and identifying key research directions to advance ST general intelligence.

==> img/taxomomy_two.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=hidden-pink!80, text=black, align=left, font=\normalsize,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
]
\begin{figure*}[!t]
    \centering
    \resizebox{0.85\textwidth}{!}
    {
        \begin{forest}
            forked edges,
            for tree={
                fill=level0!80,
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\large,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=9em,font=\normalsize,fill=level1!80,}{},
            where level=2{text width=10em,font=\normalsize,fill=level2!80,}{},
            where level=3{text width=8em,font=\normalsize,fill=level3!60,}{},
            where level=4{text width=10em,font=\normalsize,fill=level4!20,}{},
            where level=5{text width=5em,font=\normalsize,}{},
            [STFMs  
                [LLM
                    [Zero-shot Learner
                        [As Augmenter
                            [ST-LLM~\cite{liu2024spatial}{,} TPLLM~\cite{ren2024tpllm}, leaf, text width=12em ]
                        ]
                        [As Predictor
                            [STEP~\cite{shao2022pre}, leaf, text width=22em]
                        ]
                        [As Agents
                            [CPPBTR~\cite{duan2019pre} {,} TFM~\cite{wang2023building}, leaf, text width=22em]
                        ]
                    ]
                    [Fine-tuning
                        [All Parameters
                            [SPGCL~\cite{li2022mining} {,} STGCL~\cite{liu2022contrastive}, leaf, text width=22em ]
                        ]
                        [Partial Parameters
                            [SPGCL~\cite{li2022mining} {,} STGCL~\cite{liu2022contrastive}, leaf, text width=22em ]
                        ]
                        [Add-on Parameters
                            [SPGCL~\cite{li2022mining} {,} STGCL~\cite{liu2022contrastive}, leaf, text width=22em ]
                        ]
                    ]
                ]
                [PFM
                    [Neural Architecture
                        [Transformer-based
                            [SPGCL~\cite{li2022mining} {,} STGCL~\cite{liu2022contrastive}, leaf, text width=22em ]
                        ]
                        [Diffusion-based
                            [SPGCL~\cite{li2022mining} {,} STGCL~\cite{liu2022contrastive}, leaf, text width=22em ]
                        ]
                        [SSM-based
                            [SPGCL~\cite{li2022mining} {,} STGCL~\cite{liu2022contrastive}, leaf, text width=22em ]
                        ]
                    ]
                    [Pre-training Schemes
                        [Generative
                            [SPGCL~\cite{li2022mining} {,} STGCL~\cite{liu2022contrastive}, leaf, text width=22em ]
                        ]
                        [Contrastive
                            [SPGCL~\cite{li2022mining} {,} STGCL~\cite{liu2022contrastive}, leaf, text width=22em ]
                        ]
                        [Hybrid
                            [SPGCL~\cite{li2022mining} {,} STGCL~\cite{liu2022contrastive}, leaf, text width=22em ]
                        ]
                    ]
                    [Data-Specific Models
                        [Location
                            [SPGCL~\cite{li2022mining} {,} STGCL~\cite{liu2022contrastive}, leaf, text width=22em ]
                        ]
                        [Trajectory/Event
                            [SPGCL~\cite{li2022mining} {,} STGCL~\cite{liu2022contrastive}, leaf, text width=22em ]
                        ]
                        [ST Graph/Raster
                            [SPGCL~\cite{li2022mining} {,} STGCL~\cite{liu2022contrastive}, leaf, text width=22em ]
                        ]
                    ]
                ]
            ]
        \end{forest}
    }    
\caption{A comprehensive taxonomy of TSFMs, categorized according to data and methodologies.}
\label{fig:taxonomy}
\end{figure*}
% , categorized according to methodologies (i.e., unconditioned vs. conditioned), tasks (e.g., predictive versus generative), and applications.
% Single-Modality
%  [xxx, leaf, text width=22em ]

% others： 展开
% 
                
